CAFE: Calar Alto Fiber-fed Echelle spectrograph

We present here CAFE, the Calar Alto Fiber-fed Echelle spectrograph, a new instrument built at the Centro Astronomico Hispano Alem\'an (CAHA). CAFE is a single fiber, high-resolution ($R\sim$70000) spectrograph, covering the wavelength range between 3650-9800\AA. It was built on the basis of the common design for Echelle spectrographs. Its main aim is to measure radial velocities of stellar objects up to $V\sim$13-14 mag with a precision as good as a few tens of $m s^{-1}$. To achieve this goal the design was simplified at maximum, removing all possible movable components, the central wavelength is fixed, so the wavelentgth coverage; no filter wheel, one slit and so on, with a particular care taken in the thermal and mechanical stability. The instrument is fully operational and publically accessible at the 2.2m telescope of the Calar Alto Observatory. In this article we describe (i) the design, summarizing its manufacturing phase; (ii) characterize the main properties of the instrument; (iii) describe the reduction pipeline; and (iv) show the results from the first light and commissioning runs. The preliminar results indicate that the instrument fulfill the specifications and it can achieve the foreseen goals. In particular, they show that the instrument is more efficient than anticipated, reaching a $S/N\sim$20 for a stellar object as faint as $V\sim$14.5 mag in $\sim$2700s integration time. The instrument is a wonderful machine for exoplanetary research (by studying large samples of possible systems cotaining massive planets), galactic dynamics (high precise radial velocities in moving groups or stellar associations) or astrochemistry.

==> LogFirstLight.tex <==
\begin{table}
\caption{Log of the First Observing night}
\label{tab:obj}      % is used to refer this table in the text
\begin{center}
\begin{tabular}{rlr}        % centered columns (4 columns)
\hline\hline                 % inserts double horizontal lines
Date & Object & Exp. Time \\
(1) & (2) & (3) \\
\hline                                   %inserts single line
2011-05-24 19:06  & Bias & 0 \\
2011-05-24 19:12  & Cont & 10 \\
2011-05-24 19:15  & Bias & 0 \\
2011-05-24 19:18  & Bias & 0 \\
2011-05-24 19:21  & Bias & 0 \\
2011-05-24 20:16  & ThAr & 30 \\
2011-05-24 20:20  & Cont & 20 \\
2011-05-24 20:25  & Cont & 5 \\
2011-05-24 20:34  & HR4728 & 5 \\
2011-05-24 20:47  & HR4728 & 5 \\
2011-05-24 21:57  & Tres-3 & 1800 \\
2011-05-24 22:13  & ThAr & 40 \\
2011-05-24 23:02  & Saturn & 100 \\
2011-05-05 23:37  & BD+26 2606 & 300\\
2011-05-25 00:26  & Tres-3 & 1800 \\
2011-05-25 01:20  & ThAr & 40 \\
2011-05-25 01:25  & Cont & 10 \\
2011-05-25 02:01  & HD192281 & 300\\
2011-05-25 02:07  & HD182488 & 100\\
2011-05-25 02:12  & HD190404 & 100\\
2011-05-25 02:32  & BD254655 & 500\\
2011-05-25 03:09  & Tres-3 & 1800\\
 \hline
\end{tabular}

(1) Date and hour in UT of the beginning of the observation; (2)
Object name; (3) Exposure time in seconds.

\end{center}
\end{table}

